On the Utility of Gradient Compression in Distributed Training Systems

A rich body of prior work has highlighted the existence of communication bottlenecks in synchronous data-parallel training. To alleviate these bottlenecks, a long line of recent work proposes gradient and model compression methods. In this work, we evaluate the efficacy of gradient compression methods and compare their scalability with optimized implementations of synchronous data-parallel SGD across more than 200 different setups. Surprisingly, we observe that only in 6 cases out of more than 200, gradient compression methods provide speedup over optimized synchronous data-parallel training in the typical data-center setting. We conduct an extensive investigation to identify the root causes of this phenomenon, and offer a performance model that can be used to identify the benefits of gradient compression for a variety of system setups. Based on our analysis, we propose a list of desirable properties that gradient compression methods should satisfy, in order for them to provide a meaningful end-to-end speedup.

==> gradcompression_amount.tex <==
\section{Amount or compression for perfect scalability ?}
Before designing gradient compression methods it will be better to evaluate how much gradient compression do we need at a given bandwidth. For this analyis we disregard encode-decode time. Our performance model enables us to analyse this quite easily. Best case scenario will be the one where we can overlap most of the communication with computation. This allows us to find approximately how much compression will lead to ideal speedup.\shivaram{can we define ideal speedup (here and before)} We simplify the performance model a bit with the assumption that whole of communication phase can be overlapped and sent in one bucket. i.e. we don't send the last bucket of gradient separately post computation. From this we get the condition for ideal speedup -
\begin{equation*}
    T_{comp} = T_{comm}(\hat{g}, p, BW)
\end{equation*}
Where $T_{comm}$ represents the time required to sync compressed gradient of size $\hat{g}$ among $p$ machines at $BW$ bandwidth. 
We assume that the compression strategy is all-reducible. This allows us to calculate the ideal value of $\hat{g}$ for at a given bandwidth $BW$, for a given number of processors $p$.
 In Figure~\ref{fig:ideal_compression} for different batch size and models we indicate the amount of gradient compression required so we see almost linear scaling for 64 machine. From this we observe that even at 10Gbps we ideally need at most $7\times$ gradient compression even for extremely small batch sizes. For larger batch sizes at 10Gbps this value goes down even further, for a communication heavy model like BERT requiring less than $2\times$ compression.
\begin{figure*}[ht]
    \begin{center}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/resnet50_ideal_compression.pdf}
    \caption{ResNet50: 64 machines}
     \label{fig:ideal_compression_resnet50}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/resnet101_ideal_compression.pdf}
    \caption{ResNet101: 64 Machines}
    \label{fig:ideal_compression_resnet101}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/vgg19_ideal_compression.pdf}
    \caption{VGG19: 64 Machines}
    \label{fig:ideal_compression_vgg19}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/bert_ideal_compression.pdf}
    \caption{BERT: 64 Machines}
    \label{fig:ideal_compression_BERT}
    \end{subfigure}
    
    \end{center}
    
    
    \caption{\small{\textbf{Amount of gradient compression for ideal speedups:} We show how much gradient compression do we need for ideal scalability with increase in bandwidth. What is interesting is at 10Gigabit  }}
    \label{fig:ideal_compression}
    \vspace{-0.2in}
\end{figure*}

\shivaram{add a takeaway here}

==> gradcompression_limit.tex <==
\section{Speedup opportunity with gradient compression}
Next we analyse how far behind is PyTorch DDP from ideal scaleup. We especially look at large batch sizes \shivaram{wehy only look at large batch sizes?}: for large batches even for communication bound model like BERT and VGG-19 we observe that the time difference between ideal scaleup and scaling provided by optimized implementations of Synchronous SGD is around 172 milliseconds per iteration at 10Gbps. \shivaram{unclear if this is a lot of time or not. Add a pointer to the earlier table with all timings} We observed that language models like BERT are significantly more communication heavy than convolution network. A gradient compression method which aims to provide meaningful speedups need to perform compression in less than the time taken by distributed data parallel in order to be relevant. \shivaram{does this match up with numbers in pipedream? and the dawnbench paper - i feel like there are lots of studies that show DDP doesn't scale well?}
\shivaram{also is there any intution on why the lines looks the way they do? why steep up at first and then slope?}

\begin{figure*}[t]
    \begin{center}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/resnet50_bsize64_ideal_compare.pdf}
    \caption{ResNet 50: Batch Size 64}
     \label{fig:ideal_resnet101_bsize64}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/resnet101_bsize64_ideal_compare.pdf}
    \caption{ResNet-101: Batch Size 64}
    \label{fig:ideal_vgg19_bsize128}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/bert_bsize12_ideal_compare.pdf}
    \caption{BERT: Batch Size 12}
    \label{fig:ideal_bert_bsize112}
    \end{subfigure}
    \end{center}
      \caption{\small{\textbf{Difference between ideal speedup and observed training speed using DDP:} We observe that for large batch sizes the }}
      \label{fig:psgd_resnet101}
    \vspace{-0.2in}
\end{figure*}
\cleanup{Add what will happen when there is }
\begin{center}\begin{minipage}{.94\linewidth}\centering
 \emph{In data center setting the difference between ideal and observed speedup is quite small at large batch sizes often less than 200 ms, giving limited opportunity for gradient compression methods to provide speedups } 

\end{minipage}\end{center}





 

==> gradcompression_speedup.tex <==
\section{Analysing speedups due to gradient compression}
In this section we analyse the utility of three popular gradient compression methods, for different number of machines. For all our experiments in this section we assume to operate on 10Gbps bandwidth (most commonly found in data center settings today). We look at three state of the art methods for gradient compression. 
\subsection{PowerSGD}
\label{sec:powersgd_speedup}
We first analyse PowerSGD~\cite{vogels2019powersgd}. PowerSGD claims to provide upto $256\times$ compression. Since PowerSGD drastically reduces gradient size, it can send the data in a single bucket.  However PowerSGD requires sending two smaller matrices namely P and Q, thus incurring twice the latency overhead. Our performance model becomes 
\begin{equation}
\begin{split}
T_{obs} \sim= T_{comp} + T_{encode-decode} + T_{comm}(P,p, BW) \\ + T_{comm}(Q,p, BW)
\end{split}
\end{equation}
Where p is the number of machines. $P$ and $Q$ are low rank matrices communicated by PowerSGD.

For ResNet50, ResNet101, VGG19 and BERT we show scalability of PowerSGD compared to Pytorch's built in Distributed Data Parallel module.
In Figure ~\ref{fig:psgd_resenet50},~\ref{fig:psgd_resnet101},~\ref{fig:psgd_vgg19}, we can clearly observe that as the batch size per machine increases DDP module ends up providing better scalability. This is because as batch size increase so does the time for backward pass which provides more opportunity to overlap computation with communication. Except in cases where the batch size per machine is very small. \shivaram{incomplete sentence? Also give some concrete numbers in the takeaway if possible} 
\begin{figure*}[t]
    \begin{center}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/resnet50_bsize16_psgd.pdf}
    \caption{ResNet50: Batch Size 16}
     \label{fig:psgd_resnet50_bsize16}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/resnet50_bsize64_psgd.pdf}
    \caption{ResNet 50: Batch Size 64}
    \label{fig:psgd_resnet50_bsize64}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/resnet50_bsize128_psgd.pdf}
    \caption{ResNet 50: Batch Size 128}
    \label{fig:psgd_resnet50_bsize128}
    \end{subfigure}
    \end{center}
    \caption{\small{\textbf{Training ResNet50 for different batch size and number of machines using PowerSGD:} We observe that for larger batch size like 64 per machine, Pytorch DDP provides better scalability because of no compression overhead and ability to overlap communication with computation}}
    \label{fig:psgd_resenet50}
    \vspace{-0.1in}
\end{figure*}

\begin{figure*}[t]
    \begin{center}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/resnet101_bsize16_psgd.pdf}
    \caption{ResNet101: Batch Size 16}
     \label{fig:psgd_resnet101_bsize16}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/resnet101_bsize32_psgd.pdf}
    \caption{ResNet101: Batch Size 32}
    \label{fig:psgd_resnet101_bsize64}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/resnet101_bsize64_psgd.pdf}
    \caption{ResNet101: Batch Size 64}
    \label{fig:psgd_resnet101_bsize128}
    \end{subfigure}
    \end{center}
      \caption{\small{\textbf{Training ResNet101 for different batch size and number of machines using PowerSGD:} We observe that for larger batch size like 64 per machine, Pytorch DDP provides better scalability because of no compression overhead and ability to overlap communication with computation}}
      \label{fig:psgd_resnet101}
    \vspace{-0.2in}
\end{figure*}



\begin{figure*}[t]
    \begin{center}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/vgg19_bsize16_psgd.pdf}
    \caption{VGG19: Batch Size 16}
     \label{fig:psgd_vgg19_bsize16}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/vgg19_bsize64_psgd.pdf}
    \caption{VGG19: Batch Size 32}
    \label{fig:psgd_vgg19_bsize64}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/vgg19_bsize128_psgd.pdf}
    \caption{VGG19: Batch Size 128}
    \label{fig:psgd_vgg19_bsize128}
    \end{subfigure}
    \end{center}
    \caption{\small{\textbf{Training VGG19 for different batch size and number of machines using:} Since VGG19 is an extremely large neural network, compression using PowerSGD significantly helps for small batch sizes}}
    \label{fig:psgd_vgg19}
    \vspace{-0.0in}
\end{figure*}

\begin{figure*}[t]
    \begin{center}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/bert_bsize8_psgd.pdf}
    \caption{BERT: Batch Size 8}
     \label{fig:psgd_bert_bsize8}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/bert_bsize10_psgd.pdf}
    \caption{BERT: Batch Size 10}
    \label{fig:psgd_bert_bsize10}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/bert_bsize12_psgd.pdf}
    \caption{BERT: Batch Size 12}
    \label{fig:psgd_bert_bsize12}
    \end{subfigure}
    \end{center}
    \caption{\small{\textbf{Training BERT for different batch size and number of machines:} Since BERT is an extremely large neural network, compression using PowerSGD significantly helps for small batch sizes}}
    \label{fig:psgd_bert}
    \vspace{-0.0in}
\end{figure*}


\subsection{TopK}
\label{sec:topk_speedup}
Sending Top K\% of gradients by absolute value is one of the very popular methods, we observe that high encode-decode time and lack of all-reducibility makes Topk extremely slow and not scalable. For TopK the performance model becomes 
\begin{equation*}
\begin{split}
T_{obs} \sim= T_{comp} + T_{encode-decode}+ T_{comm}(\hat{g},p, BW) \\+ T_{comm}(\hat{i}, p, BW)
\end{split}
\end{equation*}

Since TopK is not all-reducible, and we also need to send the indices, leading to twice the amount of communication, we get $_{comm}(\hat{g}) = \frac{\hat{g} \times (p-1)}{BW}$, where $\hat{g}$ is the bucket size, p is the number of machines. Exact same amount of communication will be incurred for communicating the indices. 
We provide results for Topk on ResNet-50 in Figure~\ref{fig:topk_resnet50}.  Additional results on ResNet101 and VGG19 can be found in Appendix~\ref{sec:additional_results}. 
\shivaram{can we summarize these graphs in one number. Something like Top-K performs well up to X or DDP performs better up to X and then TOP-K has Z\% win}

\begin{figure*}[t]
    \begin{center}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/resnet50_bsize16_topk.pdf}
    \caption{ResNet50: Batch Size 16}
     \label{fig:topk_resnet50_bsize16}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/resnet50_bsize64_topk.pdf}
    \caption{ResNet 50: Batch Size 64}
    \label{fig:topk_resnet50_bsize64}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/resnet50_bsize128_topk.pdf}
    \caption{ResNet 50: Batch Size 128}
    \label{fig:topk_resnet50_bsize128}
    \end{subfigure}
    \end{center}
    \caption{\small{\textbf{Training ResNet50:} We compare total runtime of TopK for K when compared to using an optimized implementation of Synchronous SGD }}
    \label{fig:topk_resnet50}
    \vspace{-0.0in}
    \end{figure*}

\subsection{SignSGD}
\label{sec:signsgd_speedup}
SignSGD is another popular technique for performing gradient compression. In this case SignSGD only sends 1bit for each 32bit leading to around $32\times$  gradient compression. Although SignSGD is extremely quick to decode and encode we observe that due to lack of all reducibility it's communication time increases linearly.
Moreover SignSGD at best can provide $32\times$ compression which is not enough to offset the lack of all reducibility.
\begin{equation*}
\begin{split}
T_{obs} \sim= T_{comp} + T_{encode-decode}+ T_{comm}(\hat{g},p, BW) 
\end{split}
\end{equation*}
$T_{comm}(k,b,p) = k\times(\frac{b\times (p-1)}{BW})$
In Figure~\ref{fig:signsgd_resnet50} we show that training ResNet-50 with SignSGD doesn't scale  well when compared to using DDP. For scalability results on ResNet101 and VGG19 we refer the reader to Appendix~\ref{sec:additional_results}.
\shivaram{can we summarize the graphs in the appendix with one number. Something like Top-K performs well up to X or DDP performs better up to X and then TOP-K has Z\% win}

\begin{figure*}[ht]
    \begin{center}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/resnet50_bsize16_signsgd.pdf}
    \caption{ResNet50: Batch Size 16}
     \label{fig:signsgd_resnet50_bsize16}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/resnet50_bsize64_signsgd.pdf}
    \caption{ResNet 50: Batch Size 64}
    \label{fig:signsgd_resnet50_bsize64}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/resnet50_bsize128_signsgd.pdf}
    \caption{ResNet 50: Batch Size 128}
    \label{fig:signsgd_resnet50_bsize128}
    \end{subfigure}
    \end{center}
    \caption{\small{\textbf{Training ResNet50:} We compare total runtime of SignSGD compared to using an optimized implementation of Synchronous SGD }}
    \vspace{-0.0in}
    \label{fig:signsgd_resnet50}
    \end{figure*}
    
\begin{center}\begin{minipage}{.94\linewidth}\centering
 \emph{Gradient Compression methods often lead to higher per iteration time. This is due to high encode-decode overhead and incompatibility with all-reduce based collection.} 
 \shivaram{lets be more precise than "often"? Maybe something about num machines or batch size?}

\end{minipage}\end{center}

